An Integer Programming Model for Embedding Social Values into Software Requirement Selection

The existing software requirement selection methods have mainly focused on optimizing the economic value of a software product while ignoring its social values and their long-term impacts on the society. Social values however, are also important and need to be taken into account in software requirement selection. Moreover, social values of software requirements may change in the presence or absence of other requirements due to the value dependencies among those requirements. These dependencies are imprecise and hard to specify in software projects. This paper presents an Integer Programming (IP) model for the integration of social values and dependencies among them into software requirement selection. We further, account for the imprecision of social values and dependencies among them using the algebraic structure of fuzzy graphs.

==> selection_ilp.tex <==
\subsection{The Integer Linear Programming Model}
\label{sec_factoring_dars}

\textcolor{red}{This section presents} our proposed integer linear programming (ILP) model for optimizing the overall value of a software product. Overall value of a requirement subset, as given by (\ref{eq_ch_dars_ov}), considers user preferences and the impacts of value dependencies on the expected values of the selected requirements. The proposed ILP model hence embeds user preferences and value dependencies into requirement selection by optimizing the overall value of a software product.  

Equations (\ref{Eq_ch_dars_dars})-(\ref{Eq_ch_dars_dars_c5}) give our proposed integer programming model as a main component of the DARS-ILP method. In these equations, $x_i$ is a selection variable denoting whether a requirement $r_i$ is selected ($x_i=1$) or ignored ($x_i=0$). Also $\theta_i$ in (\ref{eq_ch_dars_penalty}) specifies the penalty of a requirement $r_i$, which is the extent to which the expected value of $r_i$ is impacted by ignoring (selecting) requirements with positive (negative) influences on the value of $r_i$. Constraint~(\ref{Eq_ch_dars_dars_c2}) on the other hand accounts for precedence dependencies among requirements and the value implications of those dependencies. 

\begin{align}
\label{Eq_ch_dars_dars}
& \text{Maximize } \sum_{i=1}^{n} x_i (1-\theta_i) E(v_i)\\[5pt]
\label{Eq_ch_dars_dars_c1}
&\text{Subject to} \sum_{i=1}^{n} c_i x_i \leq b\\[5pt] 
\label{Eq_ch_dars_dars_c2}
& \begin{cases}
x_i \le x_j  & r_j \text{ precedes } r_i \\[5pt]
x_i \le 1-x_j& r_i \text{ conflicts with } r_j,\text{ }i\neq j= 1,...,n\\[5pt]
\end{cases}\\[5pt]
\label{Eq_ch_dars_dars_c3}
& \theta_{i} \geq \bigg(\frac{\lvert I_{i,j} \rvert + (1-2x_j)I_{i,j}}{2}\bigg),& i\neq j = 1,...,n\\[5pt]
\label{Eq_ch_dars_dars_c4}
&\text{ }x_i \in \{0,1\},& i = 1,...,n \\[5pt]
\label{Eq_ch_dars_dars_c5}
&\text{ } 0 \leq \theta_i \leq 1,& i = 1,...,n
\end{align}

Moreover, for a requirement $r_i$, $\theta_i$ depends on the selection variable $x_j$ and the strength of positive (negative) value dependencies as given by~(\ref{eq_ch_dars_penalty}). Since $I_{i,j}$ is computed by (\ref{Eq_ch_dars_influence}), prior to the optimization process, we can write $\theta_i$ as a function of $x_j$: $\theta_i=f(x_j)$. The objective function~(\ref{Eq_ch_dars_dars}), thus, can be restated as $\text{Maximize } \sum_{i=1}^{n} x_i E(v_i) - x_if(x_j)E(v_i)$ where $x_if(x_j)E(v_i)$ is a quadratic non-linear expression~\cite{boyd2004convex}. Equations (\ref{Eq_ch_dars_dars})-(\ref{Eq_ch_dars_dars_c3}), on the other hand, denote a convex optimization problem as the model maximizes a concave objective function with linear constraints. 

\begin{align}
\label{Eq_ch_dars_dars_linear}
&\text{Maximize }  \sum_{i=1}^{n} x_i E(v_i) - y_i E(v_i)\\[5pt]
\label{Eq_ch_dars_dars_linear_c1}
&\text{Subject to} \sum_{i=1}^{n} c_i x_i \leq b\\[5pt]
\label{Eq_ch_dars_dars_linear_c2}
& \begin{cases}
x_i \le x_j  & r_j \text{ precedes } r_i \\[5pt]
x_i \le 1-x_j& r_i \text{ conflicts with } r_j,\text{ }i\neq j= 1,...,n
\end{cases}\\[5pt]
\label{Eq_ch_dars_dars_linear_c3}
& \theta_{i}\geq \bigg(\frac{\lvert I_{i,j} \rvert + (1-2x_j)I_{i,j}}{2}\bigg),& i\neq j = 1,...,n\\
\label{Eq_ch_dars_dars_linear_c4}
& -g_i \leq x_i \leq  g_i,& i=1,...,n\\[5pt]
\label{Eq_ch_dars_dars_linear_c5}
& 1-(1-g_i) \leq x_i \leq 1+(1-g_i),& i=1,...,n\\[5pt]
\label{Eq_ch_dars_dars_linear_c6}
& -g_i \leq y_i \leq g_i,& i=1,...,n\\
\label{Eq_ch_dars_dars_linear_c7}
& -(1-g_i)\leq(y_i-\theta_i) \leq (1-g_i),& i=1,...,n\\[5pt]
\label{Eq_ch_dars_dars_linear_c8}
&\text{ } 0 \leq y_i \leq 1,& i = 1,...,n\\[5pt]
\label{Eq_ch_dars_dars_linear_c9}
&\text{ } 0 \leq \theta_i \leq 1,& i = 1,...,n \\[5pt]
\label{Eq_ch_dars_dars_linear_c10}
& \text{ }x_i,g_i \in \{0,1\},& i=1,...,n
\end{align}

Convex optimization problems are solvable~\cite{boyd2004convex}. However, for problems of moderate to large sizes, Integer Linear programming (ILP) models are preferred~\cite{luenberger2015linear} as they can be efficiently solved, despite the inherited complexity of NP-hard problems, due to the advances in solving ILP models and availability of efficient tools such as ILOG CPLEX for that purpose. This motivates us to consider developing an ILP version of the model as given by~(\ref{Eq_ch_dars_dars_linear}). 

In doing so, non-linear expression $x_i\theta_i$ is substituted with the linear expression $y_i$ ($y_i=x_i\theta_i$). As such, either $a:(x_i=0,y_i=0)$, or $b:(x_i=1,y_i=\theta_i)$ occur. To capture the relation between $\theta_i$ and $y_i$ in a linear form, we have made use of an auxiliary variable $g_i=\{0,1\}$ and (\ref{Eq_ch_dars_dars_linear_c4})-(\ref{Eq_ch_dars_dars_linear_c8}) are added to the original model. As such, we have either $(g_i=0) \rightarrow a$, or $(g_i=1) \rightarrow b$. The resulting selection model as given by~(\ref{Eq_ch_dars_dars_linear})-(\ref{Eq_ch_dars_dars_linear_c10}) is an integer linear model. 

% Example was commented out as we r presenting a case study and btw example can not show how selection algorithm works! all conclusions can be drawn form case study and sim results
%\begin{exmp}
%\label{ex_dars}
%Consider finding the optimal subset of requirements of Example~\ref{ex_fuzzy_relation} with value dependency graph $G=(R,\sigma,\rho)$ as given by Figure \ref{fig_ex_vdg} where a release budget of $Budget=25$ is available. Also, costs and customer values of requirements are estimated as $C=\{10,10,15,10\}$ and $V=\{20,10,50,10\}$ respectively. Table~\ref{table_ex_all} lists all subsets of requirements of $R$ referred to as candidate solutions. Each candidate solution in Table~\ref{table_ex_all} is denoted by a solution vector $X_k=\{x_1,x_2,x_3,x_4\}$ in which $x_i$ specifies whether the requirement $r_i$ is selected ($x_i=1$) or ignored ($x_i=0$). Also, for each solution $X_k$ a penalty vector $\theta_k=\{\theta_1,\theta_2,\theta_3,\theta_4\}$ denotes penalties of selected requirements where $\theta_i$ specifies the penalty of requirement $r_i$ calculated by Equation~(\ref{Eq_ch_dars_penalty}). For a candidate solution $X_k$ accumulated cost (AC)/accumulated customer value  (ACV) of $X_k$ are calculated by accumulating the costs/customer values of selected requirements in $X_k$ as listed in Table~\ref{table_ex_all}. Also, overall customer value (OCV) of each candidate solution is calculated by Equation(\ref{Eq_ch_dars_ocv}) and listed in Table~\ref{table_ex_all}.  
%-----------------------------------------------------------
%\begin{table*}[t]
%	\caption{Global caption}
%	\caption{Candidate solutions for Example~\ref{ex_dars}}
%	\label{table_ex_all}
%	\centering
%	\input{tables/table_ex_all}
%\end{table*}
%-------------------------------------------------------------
%\textit{DARS} model as given by Equations~(\ref{Eq_ch_dars_dars_linear})-(\ref{Eq_ch_dars_dars_linear_c7}) finds a subset of requirements with the highest overall customer value ($OCV)$ while keeping the \textit{accumulated cost (AC)} within the budget ($\sum_{i=1}^{n}x_ic_i \leq 25$). It is clear form Table~\ref{table_ex_all} that among all the candidate solutions with $AC\leq 25$, $X_{10}=\{0,0,1,1\}$ with $OCV(X_{12})=28$ yields the highest overall customer value. Therefore, $X_{12}$ will be selected as the optimal set by $DARS$ model. 
%
%When a \textit{BKP} model is employed to find the optimal set for the given example, it will select the candidate solution $X_5=\{1,0,1,0\}$ which gives the highest \textit{accumulated customer value} ($ACV(X_5)=70$) while keeping the cost within the budget ($AC(X_6)\leq Budget$). However, \textit{BKP} models' selected solution ($X_6$) does not give the maximum \textit{overall customer value} among the feasible solutions($OCV(X_5)<OCV(X_6)<OCV(X_12)$). 
%
%A \textit{BKP-PC} model on the other hand will select a solution with the highest \textit{accumulated customer value} while considering the precedence constraints among the requirements. As discussed earlier, not all of the value dependencies are determined by \textit{Precede} relations. However, \textit{BKP-PC} model can only capture value dependencies that are determined by \textit{Precede} relations. Hence, we have to formulate value dependencies of the present example as precedence constraints when a \textit{BKP-PC} model is employed. For instance, we can derive precedence constraint $x_1 \leq x_2$ from $\sigma_{1,2}=+$. Also can derive precedence constraint $x_1 \leq 1-x_2$ from $\sigma_{1,2}=-$. In a similar way all of the precedence constraints of the \textit{BKP-PC} model for the present example are identified and listed in Table~\ref{table_ex_dars_constraints}. From constraints $x_1\leq x_2$ and $x_1\leq 1-x_2$ we can infer that $x_1\leq \frac{1}{2}$. On the other hand we have $x_1 \in \{0,1\}$. Therefore, $ x_1=0$. In a similar way it can be inferred from $x_3 \leq x_4$ and $x_3 \leq 1-x_4$ that $x_3=0$. Also from $x_1=x_3=0$, $x_2 \leq x_1$ and $x_4 \leq x_3$ we can conclude that $x_2=x_4=0$. Therefore, it is not possible to satisfy the constraints of Table~\ref{table_ex_dars_constraints} unless all of the requirements are ignored ($x_1=x_2=x_3=x_4$). Therefore, a \textit{BKP-PC} model will select $X_0$ in Table~\ref{table_ex_all} with $ACV = OCV = 0$ as the optimal solution. In other words, a \textit{BKP-PC} does not select any of the requirements of the present example even though budget is available for some of those requirements to be implemented. This situation is referred to as \textit{Selection Deficiency Problem (SDP)} as discussed earlier.
%\end{exmp}
%
%%-------------------------------------------------------------
%\begin{table}
%	%\caption{Global caption}
%	\centering
%	\caption{Precedence constraints of \textit{BKP-PC} model for value dependencies in \textit{VDG} of Example~\ref{ex_dars}}
%	\label{table_ex_dars_constraints}
%	\input{tables/table_ex_constraints}
%\end{table}
%%-------------------------------------------------------------
%
%
%

